Are LLM-Judges Robust to Expressions of Uncertainty? Investigating the effect of Epistemic Markers on LLM-based Evaluation

In line with the principle of honesty, there has been a growing effort to train large language models (LLMs) to generate outputs containing epistemic markers. However, evaluation in the presence of epistemic markers has been largely overlooked, raising a critical question: Could the use of epistemic markers in LLM-generated outputs lead to unintended negative consequences? To address this, we present EMBER, a benchmark designed to assess the robustness of LLM-judges to epistemic markers in both single and pairwise evaluation settings. Our findings, based on evaluations using EMBER, reveal that all tested LLM-judges, including GPT-4o, show a notable lack of robustness in the presence of epistemic markers. Specifically, we observe a negative bias toward epistemic markers, with a stronger bias against markers expressing uncertainty. This suggests that LLM-judges are influenced by the presence of these markers and do not focus solely on the correctness of the content.

==> 1.intro.tex <==
\section{Introduction}
Recently, there has been growing interest in utilizing large language models (LLMs) to evaluate the performance of other LLMs~\cite{liu2023g,fu2024gptscore}. 
This approach, known as \textit{"LLM as a judge"}, is widely employed in tasks such as open-ended question answering~\cite{kamalloo2023evaluating,adlakha2024evaluating, wang2024evaluating} or the instruction following~\cite{zeng2023evaluating, jiang2023llm, jiang2023followbench}. 
Studies have shown that LLM evaluations often align well with human judgments, and due to advantages in scalability and efficiency, numerous studies have reported performance assessments of models using LLM judges~\cite{chiang2023can, wang2023chatgpt}. 

Despite its potential, several limitations of LLM-as-judge have been highlighted. 
Numerous studies have identified biases in LLM evaluations, such as verbosity, self-enhancement, and gender biases, as well as the format and cognitive biases\cite{zheng2023judging, zhu2023judgelm, chen2024humans, koo2023benchmarking}.
Also, positional bias is a particularly well-known issue, where evaluation outcomes can be influenced by the order in which comparisons are presented in pairwise settings~\cite{wang2023large, liusie2024llm}. 
Moreover, recent research highlights LLM evaluators' susceptibility to adversarial attacks, which can lead to inconsistent and unreliable results~\cite{zeng2023evaluating, raina2024llm}. 



One critical yet underexplored factor in LLM evaluation is the influence of epistemic markers—linguistic expressions that convey a speaker's confidence, certainty, or uncertainty, such as "I'm unsure", and "I'm confident" in  Figure~\ref{figure1}.
Recent studies have demonstrated that the presence of appropriate epistemic markers in model outputs significantly affects user trust~\cite{zhou2024relying, kim2024m, dhuliawala2023diachronic}, putting efforts to align LLMs with honesty standards that ensure they convey varying levels of certainty accurately~\cite{yang2023alignment, lin2022teaching, kadavath2022language}. 
As future LLMs are expected to incorporate more nuanced epistemic markers, it becomes increasingly important to develop fair evaluation systems that can handle such markers without bias.


In this paper, we address this gap by introducing EMBER, a novel benchmark designed to assess LLM evaluators' robustness to epistemic markers. 
EMBER evaluates two tasks: \textit{open-ended question answering} and \textit{instruction following}. 
Our experiments on EMBER, conducted with five LLMs, including GPT-4 and LLaMA 3 70B, reveal that LLMs struggle to maintain consistency when evaluating outputs containing epistemic markers, which undermines the reliability of their judgments. 
Specifically, we observe three key findings: (1) All LLM evaluators exhibited a bias towards epistemic markers, with weaker models being more susceptible to influence. (2) In single-scoring settings, LLMs demonstrated a negative bias toward expressions of certainty or uncertainty, with a stronger bias against uncertainty. (3) In pairwise comparisons, the impact of epistemic markers was even more pronounced, with LLM evaluators consistently favoring expressions of certainty over uncertainty.

%Additionally, we explore how epistemic markers influence pairwise evaluations of model-generated outputs in real-world scenarios. 
%Unlike EMBER, where one output is clearly correct and the other is not, real-world evaluations often involve more complexity: both outputs may be correct, only one may be accurate, or neither may fully meet the instruction. 
%This makes real-world evaluation more challenging but essential for capturing subtle distinctions in model performance. 
%Interestingly, our findings reveal that models incorporating epistemic humility—despite often producing better outputs—received unfairly lower evaluations when epistemic markers of uncertainty were present. 
%This suggests that such markers can inadvertently bias LLM evaluations, leading to misjudgments of otherwise superior outputs, particularly in nuanced scenarios.
Additionally, we analyze the impact of epistemic markers in various evaluation settings.
First, we investigate how epistemic markers influence pairwise evaluations of model-generated outputs in real-world scenarios.
After comparing outputs from weaker models (GPT-3.5) and stronger models (GPT-4 series), we introduce an uncertainty indicator to the stronger model’s output and compare them again.
Our findings reveal that models displaying epistemic humility received significantly lower evaluations when uncertainty markers were present, with GPT-3.5 outputs even outperforming a GPT-4o outputs marked with uncertainty.
Moreover, we assess whether human judges are sensitive to epistemic markers.
Unlike LLM judges, human judges exhibited robustness, highlighting the critical need to improve how LLMs evaluate outputs containing epistemic markers to ensure fair evaluations


Our contributions are threefold: \begin{itemize} \item We are the first to analyze the impact of epistemic markers in LLM-based evaluation settings. \item We propose EMBER, a meta-evaluation benchmark designed to assess the robustness of LLM evaluators in the presence of epistemic markers. \item Our experimental results show that even state-of-the-art models, such as GPT-4o, struggle to maintain robustness against epistemic markers, highlighting the need for our benchmark. \end{itemize}




%To explore the real-world implications of this lack of robustness, we examined two hypothetical scenarios. Our results suggest that in pairwise evaluations, overconfident models could gain an unfair advantage, while models expressing humility might be unfairly penalized. 
%This raises concerns about the potential for epistemic markers to be exploited as a form of manipulation in LLM-based evaluations, posing a significant challenge to the integrity of these assessment systems.


==> figure/Figure_bar.tex <==

\begin{figure*}[t]
\centering
\begin{adjustbox}{valign=t}
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/Figure_bar_fig.png}
    \end{subfigure}
    \hspace{1mm} % horizontal space between figures
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/Figure_bar_fig.png}
    \end{subfigure}
\end{adjustbox}
\vspace{1mm} % vertical space between rows
\begin{adjustbox}{valign=t}
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/Figure_bar_fig.png}
    \end{subfigure}
    \hspace{1mm}
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/Figure_bar_fig.png}
    \end{subfigure}
    \hspace{1mm}
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/Figure_bar_fig.png}
    \end{subfigure}
\end{adjustbox}

\caption{dddd}
\label{figure_bar}
%\vspace{-5mm}
\end{figure*}



==> tables/nq_result.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[t]
\renewcommand{\arraystretch}{1.3}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccccccccc}
\hline
\hline
\multicolumn{11}{c}{Natural Questions}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                              \\ \hline
\multicolumn{2}{c|}{Reader}                                                                                                                               & \multicolumn{3}{c|}{GPT-4}                                                                                                                                                               & \multicolumn{3}{c|}{ChatGPT}                                                                                                                                                             & \multicolumn{3}{c}{Newbing}                                                                                                                                        \\ \hline
\multicolumn{1}{c}{Evaluator}                      & \multicolumn{1}{c|}{Metric}                                                                         & QA\textsubscript{$\mathcal{S}$}                                                     & QA\textsubscript{$\mathcal{N}$}                                                  & \multicolumn{1}{c|}{QA\textsubscript{$\mathcal{W}$}}                                                      & QA\textsubscript{$\mathcal{S}$}                                                     & QA\textsubscript{$\mathcal{P}$}                                                  & \multicolumn{1}{c|}{QA\textsubscript{$\mathcal{W}$}}                                                      & QA\textsubscript{$\mathcal{S}$}                                                     & QA\textsubscript{$\mathcal{P}$}                                                  & QA\textsubscript{$\mathcal{W}$}                                                     \\ \hline
\multicolumn{1}{c}{\multirow{2}{*}{GPT-3.5-turbo}} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Accuracy\\ (Relative)\end{tabular}} 
& \begin{tabular}[c]{@{}c@{}}74.0\\\ (\textcolor{red}{-3.2\%})\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}77.2\\ -\end{tabular} 

& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}74.2\\ (\textcolor{red}{-3.0\%})\end{tabular}}    
& \begin{tabular}[c]{@{}c@{}}72.4\\ (\textcolor{red}{-2.8\%})\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}75.2\\ -\end{tabular} 

& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}71.8\\ (\textcolor{red}{-3.4\%})\end{tabular}}    
& \begin{tabular}[c]{@{}c@{}}71.0\\ (\textcolor{red}{-1.2\%})\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}72.2\\ -\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}72.0\\ (\textcolor{red}{-0.2\%})\end{tabular}   \\ \cline{2-11} 
\multicolumn{1}{c}{}                               & \multicolumn{1}{c|}{Absolute}                                                         
& 8.0\%                                                   
& -                                                  
& \multicolumn{1}{c|}{7.8\%}                                                    
&6.4\%                                                   
& -                                                  
& \multicolumn{1}{c|}{7.8\%}                                                    
& 9.2\%                                                   
& -                                                  
& 7.8\%                                                   \\ \hline
\multicolumn{1}{c}{\multirow{2}{*}{GPT-4-mini}}    
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Accuracy\\ (Relative)\end{tabular}} 
& \begin{tabular}[c]{@{}c@{}}82.8\\ -\end{tabular}   
& \begin{tabular}[c]{@{}c@{}}82.8\\ -\end{tabular} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}74.4
\\ (\textcolor{red}{-8.4\%})\end{tabular}}   

& \begin{tabular}[c]{@{}c@{}}79.6\\ (\textcolor{red}{-0.4\%})\end{tabular}    & \begin{tabular}[c]{@{}c@{}}80.0\\ -\end{tabular} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}70.2\\ (\textcolor{red}{-9.8\%})\end{tabular}}   
& \begin{tabular}[c]{@{}c@{}}82.4\\ -\end{tabular} & \begin{tabular}[c]{@{}c@{}}82.4\\ -\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}78.4\\ (\textcolor{red}{-4.0\%})\end{tabular} \\ \cline{2-11} 
\multicolumn{1}{c}{}                               & \multicolumn{1}{c|}{Absolute}                                                         
& 3.6\%                                                   
& -                                                  
& \multicolumn{1}{c|}{11.2\%}                                                  
& 5.2\%                                                   
& -                                                  
& \multicolumn{1}{c|}{13.8\%}                                                     
& 5.2\%                                                   
& -                                                  
& 8.4\%                                                 \\ \hline

\multicolumn{1}{c}{\multirow{2}{*}{GPT-4-turbo}}   
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Accuracy\\ (Relative)\end{tabular}} 
& \begin{tabular}[c]{@{}c@{}}84.2\\ (\textcolor{red}{-0.8\%})\end{tabular}    
& \begin{tabular}[c]{@{}c@{}}85.0\\ -\end{tabular} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}82.6\\ (\textcolor{red}{-2.4\%})\end{tabular}}  
& \begin{tabular}[c]{@{}c@{}}83.8\\ (\textcolor{blue}{+0.2\%})\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}83.6\\ -\end{tabular} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}81.4\\ (\textcolor{red}{-2.2\%})\end{tabular}}    
& \begin{tabular}[c]{@{}c@{}}84.2\\ (\textcolor{red}{-1.2\%})\end{tabular}   
& \begin{tabular}[c]{@{}c@{}}85.4\\ -\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}83.8\\ (\textcolor{red}{-1.6\%})\end{tabular}   \\ \cline{2-11} 
\multicolumn{1}{c}{}                               & \multicolumn{1}{c|}{Absolute}                                                         
& 3.6\%                                                     
& -                                                  
& \multicolumn{1}{c|}{4.8\%}                                                    
& 4.2\%                                                  
& -                                                  
& \multicolumn{1}{c|}{5.4\%}                                                    
& 3.6\%                                                   
& -                                                  
& 4.0\%                                                  \\ \hline

\multicolumn{1}{c}{\multirow{2}{*}{Llama-3-8b}}    & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Accuracy\\ (Relative)\end{tabular}} 
& \begin{tabular}[c]{@{}c@{}}80.8\\ (\textcolor{red}{-1.0\%})\end{tabular}   
& \begin{tabular}[c]{@{}c@{}}81.8\\ -\end{tabular} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}60.2
\\ (\textcolor{red}{-21.6\%})\end{tabular}}   
& \begin{tabular}[c]{@{}c@{}}78.6\\ (\textcolor{red}{-0.6\%})\end{tabular}    
& \begin{tabular}[c]{@{}c@{}}79.2\\ -\end{tabular} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}59.6\\ (\textcolor{red}{-19.6\%})\end{tabular}}   
& \begin{tabular}[c]{@{}c@{}}83.4\\ (\textcolor{red}{-1.6\%})\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}85.0\\ -\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}70.4\\ (\textcolor{red}{-14.6\%})\end{tabular} \\ \cline{2-11} 
\multicolumn{1}{c}{}                               & \multicolumn{1}{c|}{Absolute}                                                         
& 7.4\%                                                   
& -                                                  
& \multicolumn{1}{c|}{38.4\%}                                                   
& 9.4\%                                                   
& -                                                  
& \multicolumn{1}{c|}{39.2\%}                                                     
& 8.0\%                                                   
& -                                                  
& 24.2\%                                                 \\ \hline

\multicolumn{1}{c}{\multirow{2}{*}{Llama-3-70b}}    & 
\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Accuracy\\ (Relative)\end{tabular}} 
& \begin{tabular}[c]{@{}c@{}}85.2\\ -\end{tabular}   
& \begin{tabular}[c]{@{}c@{}}85.2\\ -\end{tabular} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}83.8
\\ (\textcolor{red}{-1.4\%})\end{tabular}}   
& \begin{tabular}[c]{@{}c@{}}83.8\\ (\textcolor{blue}{+0.2\%})\end{tabular}    
& \begin{tabular}[c]{@{}c@{}}83.6\\ -\end{tabular} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}82.0\\ (\textcolor{red}{-1.6\%})\end{tabular}}   
& \begin{tabular}[c]{@{}c@{}}85.0\\ (\textcolor{red}{-2.0\%})\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}87.0\\ -\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}85.0\\ (\textcolor{red}{-2.0\%})\end{tabular} \\ \cline{2-11} 
\multicolumn{1}{c}{}                               & \multicolumn{1}{c|}{Absolute}                                                         
& 3.2\%                                                   
& -                                                  
& \multicolumn{1}{c|}{7.0\%}                                                   
& 3.4\%                                                   
& -                                                  
& \multicolumn{1}{c|}{6.0\%}                                                     
& 3.6\%                                                   
& -                                                  
& 4.4\%                                                 \\ \hline
\hline

\end{tabular}%
}
\caption{QA evaluation result on correct/incorrect QA 0925 result}
\label{tab:my-table}
\end{table*}

==> tables/tq_result.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[t]
\renewcommand{\arraystretch}{1.3}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccccccccc}
\hline
\hline
\multicolumn{11}{c}{TriviaQA}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                              \\ \hline
\multicolumn{2}{c|}{Reader}                                                                                                                               & \multicolumn{3}{c|}{GPT-4}                                                                                                                                                               & \multicolumn{3}{c|}{ChatGPT}                                                                                                                                                             & \multicolumn{3}{c}{Newbing}                                                                                                                                        \\ \hline
\multicolumn{1}{c}{Evaluator}                      & \multicolumn{1}{c|}{Metric}                                                                         & QA\textsubscript{$\mathcal{S}$}                                                     & QA\textsubscript{$\mathcal{N}$}                                                  & \multicolumn{1}{c|}{QA\textsubscript{$\mathcal{W}$}}                                                      & QA\textsubscript{$\mathcal{S}$}                                                     & QA\textsubscript{$\mathcal{P}$}                                                  & \multicolumn{1}{c|}{QA\textsubscript{$\mathcal{W}$}}                                                      & QA\textsubscript{$\mathcal{S}$}                                                     & QA\textsubscript{$\mathcal{P}$}                                                  & QA\textsubscript{$\mathcal{W}$}                                                     \\ \hline
\multicolumn{1}{c}{\multirow{2}{*}{GPT-3.5-turbo}} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Accuracy\\ (Relative)\end{tabular}} 
& \begin{tabular}[c]{@{}c@{}}85.8\\ (\textcolor{red}{-3.0\%})\end{tabular}   
& \begin{tabular}[c]{@{}c@{}}88.8\\ -\end{tabular} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}84.4\\ (\textcolor{red}{-4.4\%})\end{tabular}}  
& \begin{tabular}[c]{@{}c@{}}84.8\\ (\textcolor{red}{-5.2\%})\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}90.0\\ -\end{tabular} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}84.6\\ (\textcolor{red}{-5.4\%})\end{tabular}}    
& \begin{tabular}[c]{@{}c@{}}83.6\\ (\textcolor{red}{-3.2\%})\end{tabular}   
& \begin{tabular}[c]{@{}c@{}}86.8\\ -\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}84.4\\ (\textcolor{red}{-2.4\%})\end{tabular} \\ \cline{2-11} 
\multicolumn{1}{c}{}                               & \multicolumn{1}{c|}{Absolute}                                                         
& 6.2\%                                                     
& -                                                  
& \multicolumn{1}{c|}{9.2\%}                                                      
& 7.2\%                                                  
& -                                                  
& \multicolumn{1}{c|}{9.8\%}                                                      
& 3.6\%                                                   
& -                                                  
& 4.8\%                                                 \\ \hline

\multicolumn{1}{c}{\multirow{2}{*}{GPT-4-mini}}    & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Accuracy\\ (Relative)\end{tabular}} 
& \begin{tabular}[c]{@{}c@{}}95.4\\ (\textcolor{red}{-1.4\%})\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}96.8\\ -\end{tabular} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}76.8\\ (\textcolor{red}{-20.0\%})\end{tabular}} 
& \begin{tabular}[c]{@{}c@{}}94.4\\ (\textcolor{red}{-1.4\%})\end{tabular}     
& \begin{tabular}[c]{@{}c@{}}95.8\\ -\end{tabular}   
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}74.0\\ (\textcolor{red}{-21.8\%})\end{tabular}} 
& \begin{tabular}[c]{@{}c@{}}93.2\\ (\textcolor{red}{-0.8\%})\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}94.0\\ -\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}90.2\\ (\textcolor{red}{-3.8\%})\end{tabular}   \\ \cline{2-11} 
\multicolumn{1}{c}{}                               & \multicolumn{1}{c|}{Absolute}                                                         
& 1.8\%                                                     
& -                                                  
& \multicolumn{1}{c|}{20.8\%}                                                   
& 2.6\%                                                   
& -                                                  
& \multicolumn{1}{c|}{23.0\%}                                                     
& 2.0\%                                                   
& -                                                  
& 5.0\%                                                   \\ \hline
\multicolumn{1}{c}{\multirow{2}{*}{GPT-4-turbo}}   
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Accuracy\\ (Relative)\end{tabular}} 
& \begin{tabular}[c]{@{}c@{}}97.0\\ (\textcolor{blue}{+0.2\%})\end{tabular}   
& \begin{tabular}[c]{@{}c@{}}96.8\\ -\end{tabular} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}94.4\\ (\textcolor{red}{-2.4\%})\end{tabular}}    
& \begin{tabular}[c]{@{}c@{}}95.4\\ (\textcolor{red}{-1.6\%})\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}97.0\\ -\end{tabular} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}93.4\\ (\textcolor{red}{-3.6\%})\end{tabular}}  
& \begin{tabular}[c]{@{}c@{}}95.0\\ (\textcolor{red}{-0.2\%})\end{tabular}    
& \begin{tabular}[c]{@{}c@{}}95.2\\ -\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}94.4\\ (\textcolor{red}{-0.8\%})\end{tabular} \\ \cline{2-11} 
\multicolumn{1}{c}{}                               & \multicolumn{1}{c|}{Absolute}                                                         
& 0.2\%                                                   
& -                                                  
& \multicolumn{1}{c|}{3.2\%}                                                    
& 1.6\%                                                     
& -                                                  
& \multicolumn{1}{c|}{5.6\%}                                                    
& 1.4\%                                                   
& -                                                  
& 2.0\%                                                   \\ \hline 
\multicolumn{1}{c}{\multirow{2}{*}{Llama-3-8b}}    & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Accuracy\\ (Relative)\end{tabular}} 
& \begin{tabular}[c]{@{}c@{}}90.6\\ (\textcolor{red}{-2.6\%})\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}93.2\\ -\end{tabular} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}47.8\\ (\textcolor{red}{-45.4\%})\end{tabular}} 
& \begin{tabular}[c]{@{}c@{}}92.2\\ (\textcolor{red}{-1.8\%})\end{tabular}     
& \begin{tabular}[c]{@{}c@{}}94.0\\ -\end{tabular}   
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}49.2\\ (\textcolor{red}{-44.8\%})\end{tabular}} 
& \begin{tabular}[c]{@{}c@{}}88.6\\ (\textcolor{red}{-3.6\%})\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}92.2\\ -\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}69.0\\ (\textcolor{red}{-23.2\%})\end{tabular}   \\ \cline{2-11} 
\multicolumn{1}{c}{}                               & \multicolumn{1}{c|}{Absolute}                                                         
& 6.2\%                                                     
& -                                                  
& \multicolumn{1}{c|}{54.2\%}                                                   
& 6.6\%                                                   
& -                                                  
& \multicolumn{1}{c|}{53.6\%}                                                     
& 5.2\%                                                   
& -                                                  
& 26.0\%                                                   \\ \hline
\multicolumn{1}{c}{\multirow{2}{*}{Llama-3-70b}}    
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Accuracy\\ (Relative)\end{tabular}} 
& \begin{tabular}[c]{@{}c@{}}97.0\\ (\textcolor{blue}{+1.0\%})\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}96.0\\ -\end{tabular} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}95.0\\ (\textcolor{red}{-1.0\%})\end{tabular}} 
& \begin{tabular}[c]{@{}c@{}}97.0\\ -\end{tabular}     
& \begin{tabular}[c]{@{}c@{}}97.0\\ -\end{tabular}   
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}94.8\\ (\textcolor{red}{-2.2\%})\end{tabular}} 
& \begin{tabular}[c]{@{}c@{}}95.8\\ (\textcolor{blue}{+0.2\%})\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}95.6\\ -\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}95.6\\ -\end{tabular}   \\ \cline{2-11} 
\multicolumn{1}{c}{}                               & \multicolumn{1}{c|}{Absolute}                                                         
& 1.0\%                                                     
& -                                                  
& \multicolumn{1}{c|}{4.2\%}                                                   
& -                                                   
& -                                                  
& \multicolumn{1}{c|}{3.4\%}                                                     
& 0.6\%                                                   
& -                                                  
& 1.2\%                                                  \\ \hline
\hline

\end{tabular}%
}
\caption{QA evaluation result on correct/incorrect QA 0925 result}
\label{tab:my-table}
\end{table*}
